Detecting AI Trojans Using Meta Neural Analysis

In machine learning Trojan attacks, an adversary trains a corrupted model that obtains good performance on normal data but behaves maliciously on data samples with certain trigger patterns. Several approaches have been proposed to detect such attacks, but they make undesirable assumptions about the attack strategies or require direct access to the trained models, which restricts their utility in practice. This paper addresses these challenges by introducing a Meta Neural Trojan Detection (MNTD) pipeline that does not make assumptions on the attack strategies and only needs black-box access to models. The strategy is to train a meta-classifier that predicts whether a given target model is Trojaned. To train the meta-model without knowledge of the attack strategy, we introduce a technique called jumbo learning that samples a set of Trojaned models following a general distribution. We then dynamically optimize a query set together with the meta-classifier to distinguish between Trojaned and benign models. We evaluate MNTD with experiments on vision, speech, tabular data and natural language text datasets, and against different Trojan attacks such as data poisoning attack, model manipulation attack, and latent attack. We show that MNTD achieves 97% detection AUC score and significantly outperforms existing detection approaches. In addition, MNTD generalizes well and achieves high detection performance against unforeseen attacks. We also propose a robust MNTD pipeline which achieves 90% detection AUC even when the attacker aims to evade the detection with full knowledge of the system.

==> body/backup/approach.tex <==




%In this section, we will talk about our technique for detecting AI Trojans, which we call \emph{Meta Neural Analysis}. 
In this section, we propose a novel approach for analyzing neural networks, which we call \emph{Meta Neural Analysis}.
An overview of the workflow of our approach is shown in xx.\TODO{Add the workflow figure}
We borrow the idea from membership inference \cite{shokri2017membership} to look into the input-output pair of the model, and from property inference attack \cite{ganju2018property} to train shadow models and build a meta classifier over them.



\subsection{Shadow Models and Meta Classifier}
% In \cite{ganju2018property}, the authors propose a shadow-models-meta-classifier pipeline for property inference attack: in order to judge whether a model has some property or not, they first train a set of similar models (the shadow models) with and without that property. They then develop a meta classifier which takes a model as input and classify whether the model has property or not. After they train the meta classifier over the shadow models, they can feed the target model into the meta classifier and judge whether or not it has the property.

% We use this pipeline in this work. In particular, since we assumed that the consumer has a dataset of his own, he could train the shadow models with or without the attack approaches based on his own dataset. Then he could train a meta classifier using these shadow models to classify whether a model suffers from Trojan attacks. 

In order to analyze the internal property of a specific neural network, we borrow the idea from \cite{ganju2018property} that we can first generate some shadow models which is similar to the given neural network. The shadow models are trained by ourselves (e.g. using self-collected or reversely engineered data) so we know about its property. Then we can train a meta analyzer which learns to analyze neural networks properties from the shadow models. Usually we focus on binary analysis results (e.g. whether the model contains Trojans), so the meta analyzer is itself a machine learning binary classification model which takes a network as input and output a binary prediction. We mainly focus on this type of meta classifier in this paper and it is natural to extend it to more general classification or regression tasks.

Therefore, the pipeline goes like this: we first train a number of shadow models $\text{NN}(x)$ with and without some internal property and get a dataset $\{(\text{NN}_1, b_1), \ldots, (\text{NN}_M, b_M)\}$, where $b_i$ is the binary label for the network. Next, we build a meta classifier which extracts information from the models and use the information to predict whether the model contains the Trojan. We train the meta classifier using the shadow models and its corresponding labels. Finally, we can use the meta classifier to analyze the property of the provided model.

The meta classifier proposed in \cite{ganju2018property} is simply based on the parameters in a fully connected neural network. This architecture cannot meet the need for the various neural networks used in practice (e.g. convolutional neural network) and application scenario (e.g. only black-box access is allowed).
Therefore, we are going to propose our architecture for the meta classifier, which we call \emph{Meta Neural Analysis}. We will first introduce the most straightforward meta classifier which supports partial black-box access to the model (Section \ref{sec:outnn}). Then we will propose an improved model if we have white-box access to the model (Section \ref{sec:embnn}).
Finally we will introduce a framework to use Meta Neural Analysis for novelty detection (Section \ref{sec:one-class}), which shows the flexibility of our approach.
%Finally we will talk about the case when the consumer does not know the attack approach (Section \ref{sec:one-class}) or when the consumer has complete black-box access to the model (Section \ref{sec:transfer}).

\subsection{Output-based Meta Classifier}
\label{sec:outnn}

The key problem for the meta classifier is how to extract information and how to make predictions. We use a way similar to that used in membership inference attack \cite{shokri2017membership} to get information from neural networks: feed input into neural networks and examine its output to extract useful information. Intuitively, models with different properties will behave differently on some input data. Therefore, we can separate models with different properties as long as we find a good classification model and a proper input set.
%Intuitively, this approach is effective in judging whether a model has suffered from Trojan attack - if we feed some input with the Trojan trigger into the Trojaned model, it will produce significantly different output compared with that produced by benign models. Hence, we can use the output vectors to judge whether the model contains malicious Trojan.

In particular, consider a set of input $\{{\bf x}_1, \ldots, {\bf x}_N\}$ where ${\bf x}_i \in \mathbb{R}^{d_x}$ (for simplicity we assume that the input is a $d_x$-dimensional vector and it can easily generalize to other input spaces such as the $W\times H$ RGB image data space $\mathbb{R}^{3\times W \times H}$). Consider the neural network model for a $C$-way classification task ${\bf y}=\text{NN}({\bf x}) \in \mathbb{R}^{C}$, where the $c$-th element in $\bf y$ corresponds to the confidence score that ${\bf x}$ belongs to the $c$-th class. We will feed the $N$ inputs into the neural network and get the $N$ output vectors ${\bf y}_1, \ldots, {\bf y}_N$. By concatenating all the output vectors together, we got a representation vector $y_{model}$ for the model:
\begin{equation}
    {\bf y}_{model} = [[{\bf y}_1 || \ldots || {\bf y}_N]] \in \mathbb{R}^{CN}
\end{equation}
where $[[\cdot||\cdot||\cdot]]$ stands for the concatenation operation. The meta-classifier will then use $y_{model}$ as input and apply a binary classifier to classify the property of the model. In practice, we use a two layer neural-network as the binary classifier:
\begin{equation}
    \label{eqn:meta}
    \text{META}({\bf y}_{model};\theta) = {\bf w}^\intercal \text{ReLU}( V\cdot {\bf y}_{model})
\end{equation}
where $V \in \mathbb{R}^{H\times CN}$ and ${\bf w} \in \mathbb{R}^{H}$ are the parameters in the classifier, $\theta=\{V, {\bf w}\}$ denotes the parameters and $H$ is the hidden layer size and $\text{ReLU}(x)=\max(x,0)$ is the non-linear activation function. The output $\text{META}({\bf y}_{model};\theta)$ indicates the confidence score that the shadow model has a certain property.

The problem left is how to choose the input set $\{{\bf x}_1, \ldots, {\bf x}_N\}$ and how to train the meta classifier. The simplest choice is to randomly sample and fix some input from the input space. Then the training process is as following: given the set of shadow classifiers and corresponding labels $\{(\text{NN}_1, b_1), \ldots, (\text{NN}_M, b_M)\}$, we for each model calculate its representation vector and then optimize the loss of the binary classifier:
\begin{equation}
    \argmin_{ \theta } \sum_{j=1}^M L\Bigg(\text{META}\Big([[\text{NN}_j({\bf x}_1) || \ldots || \text{NN}_j({\bf x}_N)]];\theta\Big), b_j\Bigg)
\end{equation}

However, in practice we found that the randomly sampled input set does not work well. We would like the input to be some special ones which could lead to the most different behavior between models with different properties. Hence, our solution is to jointly optimize the chosen input and the meta binary classifier. That is to say, we include the input set in the optimization parameters and the optimization problem becomes:
\begin{equation}
    \label{eqn:loss}
    \argmin_{ \substack{\theta \\ \{{\bf x}_1, \ldots, {\bf x_N}\}}} \sum_{j=1}^M L\Bigg(\text{META}\Big([[\text{NN}_j({\bf x}_1) || \ldots || \text{NN}_j({\bf x}_N)]];\theta\Big), b_j\Bigg)
\end{equation}

The entire process is differentiable: we feed the input vectors into the shadow models and use their output as the input values for the meta classifier where both shadow models and the meta classifier is differentiable. Hence, we can directly calculate the gradient of the loss with respect to the input vectors ${\bf x}_1, \ldots, {\bf x}_N$. Therefore, we can still use the standard gradient-based optimization technique for solving Eqn. \ref{eqn:loss}.

Note that during the training process we need to access the internal parameters of the shadow models for calculating the gradient. However, this does not violate the partial black-box setting because the shadow models are trained by us and we can for sure access their parameters. During the inference process, we only need to query the provided model with ${\bf x}_1, \ldots, {\bf x}_N$ and use the output for prediction. Therefore, the entire pipeline works under the partial black-box setting. We call this pipeline \emph{Output-based Meta Classifier}.



\subsection{One-class Meta Neural Analysis}
\label{sec:one-class}
%Now we consider a more difficult Trojan detection scenario: we do not know what attack approach the attacker may use. Hence, we cannot train shadow models with Trojan for training the meta classifier. Nevertheless, in partial black-box setting we can train benign shadow models without Trojan. Therefore, the task becomes a novelty detection problem, i.e., finding test data that are different from data used during training process. We refer to this situation the \emph{one-class Scenario}.
The Meta Neural Analysis approach can not only handle the standard binary classification task over neural networks, but also adapt to different tasks such as novelty detection over neural networks. Under this setting, we assume that we can only train shadow classifiers with a specific property. Then we are required to predict whether a provided neural network has that property or not.

% We adopt the \emph{one-class neural network} approach as proposed in \cite{chalapathy2018anomaly}, which generalize the idea of one-class SVM model \cite{manevitz2001one}. 
One standard approach for performing novelty detection on data points in Euclidean place is the one-class SVM model \cite{manevitz2001one}. The One-class SVM model trains a hyper-plane which separates all the training data from the origin while maximizing the distance from the origin to the hyper-plane. Given a linear classifier $f({\bf x})={\bf w}^\intercal{\bf x}$ and a training set $\{{\bf x}_i\}$, the optimization problem is:
\begin{equation}
    \label{eqn:ocsvm}
    \min_{{\bf w}, \rho} \frac12 ||{\bf w}||_2 + \frac1\nu\cdot\frac1N\sum_{i=1}^N \text{ReLU}\big(\rho - f({\bf x_i})\big) - \rho
\end{equation}
where $\nu\in(0,1)$ is the hyper-parameter controlling the allowed false positive ratio. Standard SVM solver can be used to solve the optimial $\bf w$ and $\rho$.

In order to perform novelty detection over neural networks, we refer to the approach as in  \cite{chalapathy2018anomaly} which shows that this one-class optimization goal can be generalized to neural networks. The optimization goal is similar to Eqn.\ref{eqn:ocsvm} except that the term $||{\bf w}||_2$ becomes the Frobenius norm of all the parameters in the network. In order to solve the optimization problem, \cite{chalapathy2018anomaly} proposes to alternatively optimize the parameters in $NN$ and the radius $\rho$. The parameters are optimized using gradient-based approach and the optimal radius $\rho$ can be analytically calculated given the model $NN$. 

In our case, we first train a number of shadow models with the specific property. Then we fit a meta model using the one-class optimization goal. Note that the entire pipeline is still differentiable. So when we optimizing the parameters of the meta classifier, we also optimize the goal w.r.t. the chosen input set using the same gradient-based approach. Therefore, the optimization problem becomes:
\begin{equation}
    \label{eqn:ocnn}
    \min_{\substack{f, \rho\\ \{{\bf x}_1, \ldots, {\bf x_N}\}}} \frac12\cdot\text{l2\_losses}(\text{META}) + \frac1\nu\cdot\frac1N\sum_{i=1}^N \text{ReLU}\big(\rho - f({\bf x_i})\big) - \rho
\end{equation}
where $\text{l2\_losses}(f)$ stands for the Frobenius norm of all the parameters in the network. After we train the one-class meta-classifier, we can use it to predict whether a target model belongs to the benign class or not.



% Given a neural network model $f$ and the training set, the optimization problem becomes:
% \begin{equation}
%     \label{eqn:ocnn}
%     \min_{f, \rho} \frac12\cdot\text{l2\_losses}(f) + \frac1\nu\cdot\frac1N\sum_{i=1}^N \text{ReLU}\big(\rho - f({\bf x_i})\big) - \rho
% \end{equation}
% $\text{l2\_losses}(f)$ stands for the Frobenius norm of all the parameters in the network. For example, for the two-layer binary neural network in Eqn. \ref{eqn:meta}, the l2-loss will be $||{\bf w}||_2 + ||V||_F$. In order to solve the optimization problem, \cite{chalapathy2018anomaly} proposes to alternatively optimize the parameters in $NN$ and the radius $\rho$. The parameters are optimized using gradient-based approach and the optimal radius $\rho$ can be analytically calculated given the model $NN$. 

% In our case, we first train a number of shadow models without Trojan. Then we train a meta classifier (either output based or feature-based) using the goal in Eqn.\ref{eqn:ocnn}. Note that the entire pipeline is still differentiable. So when we optimizing the parameters of the meta classifier, we also optimize the goal w.r.t. the chosen input set using the same gradient-based approach. After we train the model, we can use it to predict whether the provided model is a novelty (i.e. malicious) or not.



==> body/backup/approach_prev.tex <==

\subsection{Meta-classifier over Neural Networks}
The main pipeline of our inference attack is similar to that proposed in \cite{ganju2018property}. Suppose the adversary is interested in deciding whether the model producer has property $P$ or does not have property $P$ (i.e., $\overline{P}$). Our intuition is that the neural network models with property $P$ will exhibit a different pattern compared to the models without it. The adversary would like to discover this pattern and distinguish between models with $P$ and $\overline{P}$. Therefore, the adversary will use another machine learning model to do this classification task and we call it the `meta classifier'. That is, a meta classifier will take a neural network as input and predict whether or not the network has property $P$.

In order to train the meta classifier, the adversary will need to train many neural networks with and without property $P$ using his own dataset, and use these neural network models as the training data for the meta-classifier. We call these models the `shadow models' trained by the adversary. Note that although the adversary's dataset is not the same as the one from the producer, the datasets still follow the same distribution and thus we could expect that the shadow model shows the similar pattern as the provider's model. In Scenarios-3, however, the adversary may not know exactly what $P$ is, so he only has the shadow models with property $\overline{P}$. Hence, he need to fit a novelty detection model from his shadow classifiers and infer about the producer's model. We will talk about this novelty detection approach in Section \ref{sec:one-class}. 

The simplest structure for the meta classifier is a fully-connected neural network over all the parameters in the original neural network. But as shown in \cite{ganju2018property}, this approach does not work well because of the large number of parameters in the meta classifier and thus it is hard to fit a good model. We are going to propose several approaches in the following, which would improve the performance of meta classifier and work in different scenarios, e.g. in black-box scenario where the adversary has no access to the model parameters.

\subsection{Parameter-based Embedding for Fully-Connected Neural Networks}
Ganju et el.~\cite{ganju2018property} proposes an algorithm for meta classifier over deep neural networks based on their model parameters. The meta-classifier takes as input the parameters in each layer of the shadow model (a fully-connected neural network) and uses a neural network to predict whether the shadow model has property P or not. They recognize that neural network layers are permutation invariant - the neurons in a hidden layer can be permuted arbitrarily while the model remains equivalent. Therefore, they propose a set-based embedding technique for each layer in the FCNN.

We next describe the detailed embedding algorithm for a layer. Suppose the $k$-th fully-connected layer has input ${\bf x_{k-1}} \in \mathbb{R}^{d_{k-1}}$ and output ${\bf x_k} \in \mathbb{R}^{d_k}$. Then it calculates the output as ${\bf x_k} = W_k{\bf x_{k-1}}$, where $W_k\in\mathbb{R}^{d_k\times d_{k-1}}$ is the parameter of the layer. For simplicity we omit the bias term in the layer, since the bias can be treated as an extra column in the weight matrix. The permutation invariant means that the layer would remain equivalent when we arbitrarily permute the values in the output. Therefore, the embedding should be the same when the first dimension of $W_k$ is shuffled. So \cite{ganju2018property} adopted the set-based approach, i.e., apply transformation function $\phi$ to every row vector in $W_k$, i.e., $w_i \in \mathbb{R}^{d_{k-1}}$ and aggregate them together by taking summation $\sum_{i=1}^{d_k} \phi(w_i)$. Suppose we use a two-layer neural network as the transformation $\phi$:
\begin{equation}
\phi(x) = U_2^{(k)} \gamma(U_1^{(k)}x)
\end{equation}
where $U_1^{(k)} \in \mathbb{R}^{d_{h_1}\times d_{k-1}}$, $U_2^{(k)} \in \mathbb{R}^{d_{h_2}\times d_{h_1}}$ and $\gamma$ is the elementwise non-linear activation function. Then the embedding representation for the $k$-th layer would be:
\begin{equation}
\label{eqn:param-emb}
E_k = \sum_{i=1}^{d_k} U_2^{(k)} \gamma(U_1^{(k)} w_i)
\end{equation}

In \cite{ganju2018property}, the embedding vectors of different layers will then be concatenated together and go through a two-layer network for the prediction, i.e. whether the model has property P or not. The framework is end-to-end and the trainable parameters in the meta-classifier are $\big\{U_1^{(k)}$, $U_2^{(k)}\big\}_{k=1,2,\ldots}$ and the parameters in the final prediction part.

\subsection{Alternative View - Output-based Embedding for Fully-Connected Layers}
\label{sec:layer-out-emb}
In order to capture the equivalence of shadow classifiers, the previous approach adopt the set-based approaches for the parameters by observing the permutation invariant. There is, however, a more intuitive idea for the equivalence of shadow models: \emph{if two models are equivalent, then the outputs of them should always be the same}. Therefore, we can propose an embedding algorithm for each layer in the FCNN based on its outputs given different inputs.

In particular, consider the fully connected layer ${\bf x_k} = W_k{\bf x_{k-1}}$. Suppose we have chosen $N$ different input vectors $X^{(k)} \in \mathbb{R}^{d_{k-1} \times N}$. We can feed it through the layer and get the $N$ output $Y = W_k X^{(k)}$. Then we can calculate the embedding vector for the $k$-th layer based on $Y$. Note that the permutation invariant of neurons means that the embedding should be equivalent when permuting $Y$ at the first dimension. Therefore, we can also apply the set-based representation, i.e. first apply transformation $\phi$ to each row vector ${\bf y}_i\in \mathbb{R}^{N}$ of $Y$ and then sum them up. Therefore, the output is calculated as:
\begin{equation}
\label{eqn:layer-emb-raw}
E_k = \sum_{i=1}^{d_{k+1}}\phi({\bf y}_i)
\end{equation}

Note that ${\bf y}_i=(X^{(k)})^\intercal {\bf w}_i$. If we let $\phi(x)=U^{(k)}\gamma(x)$ where $U^{(k)} \in \mathbb{R}^{d_h\times N}$ then Eqn.\ref{eqn:layer-emb-raw} becomes
\begin{equation}
\label{eqn:laber-emb}
E_k = \sum_{i=1}^{d_{k+1}}U^{(k)}\gamma((X^{(k)})^\intercal {\bf w}_i)
\end{equation}

Then we can let $\big\{U^{(k)}, X^{(k)}\big\}_{k=1,2,\ldots}$ be the trainable parameters of the meta-classifier and train the model. Note that $X^{(k)}$ is trainable, which means that during the training process of meta-classifier, the input will also automatically change so that the chosen input can best represent the special cases of the layer to help us classify between different shadow models.

Comparing Eqn.\ref{eqn:param-emb} with Eqn.\ref{eqn:laber-emb}, we can see that the two equations are exactly the same if we let $d_{h_1}=N$, $d_{h_2} = d_h$, $U_1^{(k)}=(X^{(k)})^\intercal$ and $U_2^{(k)}=U^{(k)}$. This shows that the two framework are actually equivalent: the framework in \cite{ganju2018property} can also be interpreted as applying set-based output embedding for some selected input vectors for each layer in a fully-connected neural network. However, the latter interpretation is easier to generalize to other kinds of neural networks, such as convolutional neural networks and recurrent neural networks. On the other hand, the approach proposed in \cite{ganju2018property} can only be applied to the fully-connected networks.

\subsection{Feature-based and Prediction-based Embedding for Neural Networks}
\label{sec:nn-emb}
The framework in Section \ref{sec:layer-out-emb} computes an output-based embedding vector for each layer and concatenate them together for the inference of property P. However, it is somehow unreasonable to split the network and deal with each layer individually when we want to consider the equivalence of the entire network. For example, it is possible that two neural network models are equivalent even if none of the corresponding layers in the two models are equivalent. The representations for these two models should also be the same, but in previous architecture there is no explicit constraint that they should be equal.

Therefore, we can improve the framework by calculating the embedding vector based on the output of the entire model instead of the outputs of each layer. More specifically, consider any $c$-way classification problem from input domain ${\bf x} \in \mathbb{R}^{d_x}$ to output domain $y \in \mathcal{Y} = \{0,1,\ldots,c-1\}$. We consider the neural network models in the form:
\begin{equation}
f(X)=W\psi(X)
\end{equation}
where $\psi(X)$ processes the input into a $d_h$-dimensional feature vector by some deep non-linear transformation, and $W\in\mathbb{R}^{c\times d_h}$ is the final linear transformation that calculates the vector of prediction score of each class based on the feature vector. We propose two attack approaches for such kind of models, one based on the feature vector $\psi(X)$ and the other based on the prediction vector $f(X)$.

\paragraph{Feature-based Embedding} Suppose we have chosen $N$ different input vectors $X \in \mathbb{R}^{d_x \times N}$. We apply $\psi$ to each input vector and get the feature matrix $\Psi \in \mathbb{R}^{d_h \times N}$. Note that $\Psi$ is the last hidden layer and thus it has the property of permutation invariant. Thus, we could perform set-based transformation technique to improve the performance. We will apply set-based transformation $\phi$ to the row vectors $\psi_i$ of $\Psi$. Therefore, the embedding vector of the network can be calculated as:
\begin{equation}
E = \sum_{i=1}^{d_h} \phi(\psi_i)
\label{eqn:emb-fb}
\end{equation}
Then the embedding vector will be processed by a two-layer network and give the final prediction on property P. The trainable parameters in the framework includes $X$, parameters in $\phi$ and the parameters used in the final prediction.

\paragraph{Prediction-based Embedding} Suppose we have chosen $N$ different input vectors $X \in \mathbb{R}^{d_x \times N}$. This approach queries the neural network $N$ times and get the prediction matrix $Y \in \mathbb{R}^{c \times N}$. This prediction matrix has no permutation invariant, since the order matters in the final prediction. Therefore, we simply flatten $Y$ into a 1-d vector $Y_{flat}\in \mathbb{R}^{cN}$ and apply a transformation $\phi$, i.e.:
\begin{equation}
E = \phi(Y_{flat})
\label{eqn:emb-pb}
\end{equation}
Note that in this approach, the attacker does not need to have access to the internal parameters of the neural network during the inference stage. Therefore, this approach can work under the black-box inference attack, i.e. Scenario-2. Nevertheless, during the training process we still need to access the shadow classifiers to back-propagate the gradient, but this does not violate the black-box setting because these shadow classifiers used in training are trained by the attacker and the attacker will naturally have the access to it.

\subsection{One-class Meta classifiers}
\label{sec:one-class}
As we discussed in Section \ref{sec:problem}, in Scenario-3 the adversary may not clearly know about the target property and thus he can only get the shadow models in $\overline{P}$. Therefore, the meta classifier is a novelty detection model which is trained using shadow models with $\overline{P}$ by one-class classification techniques. After the adversary trains the meta classifier, he can apply it to the target model from the producer. The result would indicate whether the target model is with $\overline{P}$ or is an outlier (which means that it is with $P$).

Our one-class meta classifier consists of two steps: first, we will fit a model to calculate an embedding vector for each shadow model; second, we will fit a one-class SVM using all the embedding vectors of the shadow model. After we train these two models, we could make predictions on the target model. We will first use the fitted model to calculate the embedding vector for the target model. Then we can feed the embedding vector into the one-class SVM to predict whether it is an outlier case($P$) or a normal case($\overline{P}$).

The remaining question is what is the meta model for calculating embedding vector and how to train it. In practice, we try both the feature-based and prediction-based embedding technique for calculating the embedding vector as discussed in Section \ref{sec:nn-emb}. In order to train the model, we will use the shadow models with $\overline{P}$ as well as shadow models with random parameters. We train the meta model in order to distinguish between the $\overline{P}$ models and the random-valued models. After the meta model is trained, we could calculate the embedding vectors as in Equation \ref{eqn:emb-fb} (for feature-based model) or \ref{eqn:emb-pb} (for prediction-based model).

==> body/backup/threatmodel_prev.tex <==
\xiaojun{TODO}
The goal of property inference attack is to infer information from a given machine learning model which the model provider does not intend to share. Consider the case where a model producer trains a neural network for a specific task with his own dataset and model setting. The model producer may provide the model to others who also are faced with the task. However, he may not hope that his dataset or model setting will be leaked. Therefore, we are interested in discovering what information an adversary can extract given access to a trained machine learning model.

In \cite{ganju2018property}, the authors assume that the adversary has full access to the dataset and model - they have: 1) exactly the same dataset as the model provider; 2) white-box access to the model structure and parameters; 3) access to data cases both with and without the property which they would like to infer. In this work, we will restrict the knowledge of the adversary and show that an adversary can extract information with fewer knowledge. In particular, we consider the following scenario:
\begin{itemize}
	\item Scenario-1. In this scenario, the adversary's dataset is different from that of the model producer. Their datasets may follow the same distribution and may overlap in some cases, but both will have their own data cases which the other does not have. The model producer will usually have a larger dataset so that he can train a good model to share with others.
	\item Scenario-2. Same as in Scenario-1, the datasets of adversary and producer are different. Moreover, the producer only provides black-box access to the model. That is, the adversary can only query the model and get its prediction, while he cannot know the model parameters. However, we still assume that the adversary knows the model structure and training algorithm. Hence, he can train his own model using his own dataset for the inference attack.
	\item Scenario-3. Same as in Scenario-2, the datasets are different and the adversary only has black-box attack to the model. In addition, the adversary does not clearly know what the property is. For example, consider the case where a company claims that they applied some secret techniques to improve model performances. The adversary would like to see whether the company really uses some special techniques or not, but he is not clear what technique is used. Therefore, he could only base his inference on standard techniques and infer whether the company's model is similar to the standard approaches or not.
\end{itemize}

==> body/tables/comparison_eval.tex <==
\begin{table}[tbh]
    \centering
    \footnotesize
    \caption{Comparison with other Trojan detection works. \xiaojun{Move to intro?}}
    \begin{tabular}{c|c|c|c|c}
        \hline
        \multirow{2}{*}{ } & {\bf Attack} & { \bf Dataset} & {\bf Model } & {\bf Compare}\\
       & {\bf Types} & { \bf Types} & {\bf Types} & {\bf with Others} \\
        \hline
        \hline
        Our work & M, B, P & vision, speech, & CNN,  &  Yes \\
          &  & tabular, NLP & RNN &   \\
        \hline
        AC~\cite{chen2018detecting} & M & vision, NLP & CNN & No \\
        \hline
        NC~\cite{wang2019neural} & M, P & vision & CNN & No \\
        \hline
        Spectral~\cite{tran2018spectral} & M & vision & CNN & No \\
        \hline
        STRIP~\cite{gao2019strip} & M, P & vision & CNN & No \\
        \hline
        SentiNet~\cite{chou2018sentinet} & M, P & vision & CNN & No \\
        \hline
    \end{tabular}
    \label{table:eval_compare}
\end{table}

